Stay or Switch: Competitive Online Algorithms for Energy Plan Selection in Energy Markets with Retail Choice

Energy markets with retail choice enable customers to switch energy plans among competitive retail suppliers. Despite the promising benefits of more affordable prices and better savings to customers, there appears subsided participation in energy retail markets from residential customers. One major reason is the complex online decision-making process for selecting the best energy plan from a multitude of options that hinders average consumers. In this paper, we shed light on the online energy plan selection problem by providing effective competitive online algorithms. We first formulate the online energy plan selection problem as a metrical task system problem with temporally dependent switching costs. For the case of constant cancellation fee, we present a 3-competitive deterministic online algorithm and a 2-competitive randomized online algorithm for solving the energy plan selection problem. We show that the two competitive ratios are the best possible among deterministic and randomized online algorithms, respectively. We further extend our online algorithms to the case where the cancellation fee is linearly proportional to the residual contract duration. Through empirical evaluations using real-world household and energy plan data, we show that our deterministic online algorithm can produce on average 14.6% cost saving, as compared to 16.2% by the offline optimal algorithm, while our randomized online algorithm can further improve cost saving by up to 0.5%.

==> old-problem.tex <==
\section{Problem Formulation} 
\label{sec:prob} 

In this section, we present a formal mathematical model of the energy plan selection problem. In the energy market, energy retailers offer various energy plans for households to choose from. This energy plan selection problem is stated in \textbf{EPSP}, which includes households' arbitrary demands, market time-varying prices, and plan cancellation fees. Although energy plans differ around the world, they have the same main character in choosing plans. As a typical model, electricity plans offered in the US are chosen.
%We will relax this assumption in the subsequent section to incorporate more features from other countries.
Key notations are defined in Table \ref{tab:not}, and acronyms are listed in Table \ref{tab:acr}. 

\subsection{Model} 

\subsubsection{Uncertain Electricity Demands} Let the electricity demand of a household at time $t$ be $e_t$, which forms an arbitrary non-negative number sequence along timeline. Note that online algorithm design does not rely on any historical data or stochastic model of $e_t$. 

\subsubsection{Pricing Schemes} In the US, there are two major types of energy plans offered to households. Let $s_t$ be the chosen plan at time $t$, where 0 represents the fixed-rate plan and 1 represents the variable-rate plan. 

\begin{itemize} 
	\item {\em Variable-Rate Plan}: Variable-rate plans usually have relatively high costs with fluctuations according to the market. Switching to variable-rate plans do not incur any additional cost. Therefore, selecting the least-cost variable-rate plan is always the optimal among all variable-rate plans. As a result, we only need to consider one variable-rate plan at each time. Denote by $p^1_t$ the price per electricity unit for the variable-rate plan. The energy cost at time $t$ is $p^1_t\cdot e_t$. 
	
	\item {\em Fixed-Rate Plan}: Fixed-rate plans have little fluctuation compared to variable-rate plans and can be characterized by a stable ranking in a long duration. Moreover, a relatively high cancellation fee will be incurred when cancelling a fixed-rate plan. Thus we assume households not switching among fixed-rate plans. %Similarly as for variable-rate plans, there is only a single fixed rate input at each time slot.
	
	Note that a specific tiered-pricing scheme is applied to fixed-rate plans \cite{eastcoast}. Let $B_t$ be the base load for a household at time $t$, and $p^0_t$ be the price per electricity unit for the fixed-rate plan. A household pay $B_t\cdot p^0_t$ when electricity demand $e_t$ is between $0.9B_t$ and $1.1B_t$. Otherwise, under-usage fee is charged at rate $H$ when $e_t$ is less than $0.9B_t$, or over-usage fee is charged at the rate of the variable-rate plan $p_t^1$ when $e_t$ exceeds $1.1B_t$.
\end{itemize} 

\begin{table}[t] 
    \centering
	%\resizebox{\linewidth}{!} 
	\caption{Key notations.} 
	\label{tab:not} 
	\begin{tabular}{@{}c@{}| p{.35\textwidth}} 
		\toprule 
		\textbf{Notation}&\textbf{Definition}\\ 
		\midrule 
		$T$ & The total number of time intervals (unit: month)\\ 
		$\beta_t$ & The cancellation fee at time $t$ (\$)\\ 
		$\sigma_t$ & The joint input at time $t$, i.e., $\sigma_t \triangleq (e_t, p_t^0, p_t^1, B_t)$\\ 
		$s_t$ & The selected plan at time $t$ (variable-rate plan denoted by `1' and fixed-rate plan denoted by `0')\\ 
		$e_t$ & The electricity demand of customer at time $t$ (kWh)\\ 
		$p^0_t$ & The price per unit of electricity usage for fixed-rate plan (\$ / kWh)\\ 
		$p^1_t$ & The price per unit of electricity usage for variable-rate plan (\$ / kWh)\\ 
		$B_t$ & The base load for fixed-rate plan (kWh)\\ 
		$H$ & The underusage charging rate for fixed-rate plan (\$ / kWh)\\ 
		{\sffamily R} & The minimum contract length for fixed-rate plan (month)\\ 
		{\sffamily L} & The total contract length for fixed-rate plan (month)\\ 
		$\alpha$ & The cancellation fee for the residual time in the contract (\$ / month)\\ 
		\bottomrule 
	\end{tabular} 
\end{table} 

\begin{table}[t]  
    \centering
	\caption{Acronyms for problems and algorithms.} 
	\label{tab:acr} 
	\begin{tabular}{@{}c|l@{}} 
		\toprule 
		\textbf{Acronym}&\textbf{Meaning}\\ 
		\midrule 
		\textbf{EPSP} & Energy Plan Selection Problem\\ 
		\textbf{SP} & Simplified version of \textbf{EPSP}\\ 
		\textbf{dSP} & \textbf{EPSP} with linearly decreasing switching costs\\ 
		OFA$_s$ & The optimal offline algorithm for \textbf{SP}\\
		gCHASE$_s$ & Generalized version of deterministic online \\
		& algorithm CHASE$_s$ for \textbf{SP}\\
		gCHASE$_s^r$ & Randomized version of gCHASE$_s$ for \textbf{SP}\\ 
		\bottomrule 
	\end{tabular} 
\end{table} 

Define the cost function $g_t(s_t)$ based on  input $\sigma_t \triangleq (e_t, p_t^0, p_t^1, B_t)$ and the selected plan $s_t$ at time $t$ as: 
{
\begin{numcases}{g_t(s_t) \triangleq } 
\label{equ:gt} 
\begin{aligned} 
& e_t \cdot p^1_t,  & \mbox{if } s_t = 1; \\ 
& e_t \cdot p^0_t +  (p^1_t - p^0_t) \cdot (e_t - 1.1B_t)^+  \\
& \qquad \ \    + H \cdot (0.9B_t - e_t)^+,  & \mbox{if } s_t = 0.
\end{aligned} 
\end{numcases} 
}

We claim our model can be extended to describe other energy markets including Australia \cite{energymadeeasy}, as the cost function is determined only by input and the selected plan. In this paper, we focus on the US setting in \eqref{equ:gt}. 

% Now we extend this model to more advanced settings. For example, in Australia, the tariff is calculated each day, with a daily supply charge, and two types of schemes for usage \cite{energymadeeasy}: %We show the pricing of a day with $t$ counted by minutes. 
% \begin{enumerate} 
% \item {\em Tiered Tariffs}: 
% For the first $U_1$ kWh, the usage rate is $p_{\rm tier}^1$. For the next $U_2$ kWh, the usage rate is $p_{\rm tier}^2$. For the remaining part, the usage rate is $p_{\rm tier}^3$.
% \item {\em Time of Use Charges}: During peak hours, the usage rate is $p_{\rm time}^1$. During shoulder hours, usage rate is $p_{\rm time}^2$. During off-peak hours, the usage rate is $p_{\rm time}^3$.
% \end{enumerate} 

% We can also incorporate feed-in tariff from rooftop PV by modifying the cost function in (\ref{equ:gt}). %By denoting staying each scheme as a state $s_t$, and summing up the above according to their descriptions, we are able to get cost functions similar as (\ref{equ:gt}).


% Since the cost for each time $t$ is computed based on the revealed inputs and the current state of selected plan, we may suppress the exact cost formula of $g_t(s_t)$ in the decision-making process. 


\subsubsection{Cancellation Fee} When a household cancels the fixed-rate plan, a cancellation fee of the following types will incur: 
\begin{enumerate} 
	\item {\em No Fee}: The household pays zero cancellation fee but needs to inform the retailer beforehand (e.g., 30 days earlier). 
	\item {\em Constant Fee}: A fixed cancellation fee incurs when time remains in the contract belongs to certain level (e.g., \$100 if less than 12 months left in the contract, or \$200 if between 12 to 24 months left in the contract).
	\item {\em Temporally Linear-dependent Fee}: a pre-specified fee times the left period in the contract (e.g., \$10 per remaining month in the contract). 
\end{enumerate} 

Denote the cancellation fee incurred at time $t$ by $\beta_t$. We note that only one type of cancellation fee applies for each fixed-rate plan.

\subsubsection{Contract Period} There are various contracts with different contract periods and restrictions available in the market. As variable-rate plans usually charges higher than fixed-rate plans per electricity unit, most of them do not have a contract period. On the other hand, retailers aim to retain consumers in a fixed-rate plan by stipulating a long contract length. Let the minimum contract length be {\sffamily R} and the total contract length be {\sffamily L}. A household cannot quit the contract before  {\sffamily R} and need to rejoin the plan after {\sffamily L}. 

\subsection{Problem Definition} 

Divide total time period $T$ into integer slots $\mathcal{T}\triangleq\{1, \cdots, T\}$, where each slot is one month, corresponding to the minimum switching period. We aim to find a solution $\bm{s} \triangleq (s_1, s_2, \cdots, s_T)$ to the following energy plan selection problem: 
\begin{subequations} 
	\begin{align} 
	\textbf{(EPSP)\ \ } \min \  &  \ {\rm Cost}(\bm{s})\triangleq \sum_{t=1}^{T}\Big(g_t(s_t)+\hat{\beta_t}\cdot (s_t-s_{t-1})^+\Big) \label{equ:ecep-min}\\ 
	\text{subject to \ } & s_\tau \leq 1 - \bm{1}_{\{s_t<s_{(t-1)}\}} , t + 1 \leq \tau \leq t + \textsf{R} - 1, \label{equ:ecep-R}\\ 
	& \hat{\beta_t} = \bm{1}_{\{\sum_{t-\textsf{L}+1}^t s_\tau > 0\}} \cdot \beta_t, \label{equ:ecep-L}\\ 
	\text{variables \ } & s_t\in \mathcal{N}\triangleq\{0, 1\}, t\in [1,T], \notag 
	\end{align} 
\end{subequations} 
where $(x)^+ = \max\{x,0\}$ and $\bm{1}_{\{\cdot\}}$ is the indicator function. Initial state $s_0$ is 0 without loss of generality. Total cost function ${\rm Cost}(\bm{s})$ consists of operational cost $g_t(s_t)$,  which is defined in (\ref{equ:gt}), and switching cost, which incurs when cancelling the fixed-rate plan. Constraint (\ref{equ:ecep-R}) captures no cancellation during the minimum contract length of the fixed-rate plan. Constraint  (\ref{equ:ecep-L}) captures zero cancellation fee when cancelling a fixed-rate plan by the end of contract length.

\begin{align} 
     \textbf{(EPSP)\ \ }\min \  &  \ {\rm Cost}(\bm{s})\triangleq
      \sum_{t=1}^{T}\Big(g_t(s_t) +  d(s_{t-1},s_{t})\cdot I \Big)\\ 
     \text{subject to \ } 
     & d(s_{t-1},s_{t}) = \beta(s_{t-1})\cdot \bm{1}_{\{s_{t} \neq s_{t-1}\}}, \\ 
	& I = \bm{1}_{\{\sum _{i=2}^{\textsf{L}+1}|s_{t-i} - s_{t-1}| \neq 0\}}, \\ 
	\text{variables \ }  & s_t\in \mathcal{N}
	\triangleq
	\{0, 1, \cdots, n\}, t\in [1,T] \notag 
\end{align}



%\medskip

\textbf{Remarks:} Although our problem formulation is similar with the online optimization problems in LCP \cite{lcp}, CHASE \cite{chase} and their extended version \cite{oco, disc, rchase}, the fundamental difference in constraint (\ref{equ:ecep-L}) makes our problem more challenging. Note that cancellation fee depends on the last {\sffamily L} states at time $t$. Hence, we cannot follow the  sub-problem division as that of prior studies. Therefore, our problem is harder and requires non-trivial treatments.

==> random-slope.tex <==
\subsubsection{Randomized Online Algorithm}\hspace*{\fill} 

By adding randomization to an online algorithm ${\mathcal A}$, we let it make decisions probabilistically in each execution. Define the { \em expected} competitive ratio of randomized online algorihtm ${\mathcal A}$ by the smallest constant $c$ satisfying
\begin{equation}
	{\mathbb E}[{\rm Cost}_{\mathcal{A}}(s_0,\bm{\sigma})]\leq c\cdot {\rm Opt}(s_0,\bm{\sigma})+\gamma(s_0),\forall \mbox{\boldmath$\sigma$},
\end{equation}
\iffalse
\[
    {\rm CR}({\mathcal A}) \triangleq \max_{\bm{\sigma}} \frac{{\mathbb E}[{\rm Cost}({\mathcal A}[\bm{\sigma}])]}{{\rm Opt}(\bm{\sigma})},    
\]
\fi
where ${\mathbb E}[ \cdot ]$ is the expectation over all random solutions. Next, we devise a competitive randomized online algorithm for problem \textbf{SP}.

\com{Would be better to first explain Algorithm 3 before analyzing it or comparing it to other offline/online algorithms.}

Instead of changing the state at the moments when the cumulative cost difference $\Delta(t)$ already reaches 0 or $-\beta$, we introduce randomization to change the state earlier. Intuitively, when $\Delta(t)$ is observed to be approaching 0 or $-\beta$, the state should be changed in advance so that it can ``chase'' the behaviour of the optimal offline algorithm faster.
There are two aspects in judging $\Delta(t)$. One is its exact value, and the other is its changing speed. Intuitively, the closer it is to 0 (resp. $-\beta$), and the more rapidly it is increasing (resp. decreasing), the quicker the state should change to 1 (resp. 0). 

Here randomized algorithms do not necessarily entail random decisions of a single customer. When we consider an ensemble of a large number of customers using an automatic energy plan recommendation system, each customer can be given a deterministic decision rule drawn from a probabilistic ensemble of decision rules. In the end, the expected cost of a customer can be computed by the expected cost of a randomized algorithm. 

\com{At this point, the readers may not get a clear picture of the behaviors of Algorithm 3 yet, and thus they may not be able to understand the following discussion.}

\textbf{Note:} People familiar with the former randomized online algorithm rCHASE in \cite{rchase} may question why $\text{gCHASE}_s^r$ guarantees a smaller competitive ratio. We elaborate the key idea by demonstrating two examples in Figure \ref{fig:r_up_down}. The key feature in $\text{gCHASE}_s^r$ is, the probability of changing $s_t$ is affected by the relative value between $\Delta(t)$ and $\Delta(t-1)$. Figure \ref{fig:r_up_down}(a) shows that, if $\Delta(\tau)$ is greater than $\gamma_{on}$ defined in \cite{rchase}, rCHASE will change state. On the contrast, when the increment in $\Delta(t)$ is small, $\text{gCHASE}_s^r$ will not change state with high probability. Since there is small benefit 
($\Delta_1 - \Delta_0$) to gain while incurring high start-up cost ($\beta$), it is safer not changing. Similarly in \ref{fig:r_up_down}(b), rCHASE will change state whenever $\Delta(t)$ is less than $\gamma_{off}$. As the reduction in cost is determined by the decrement at this time ($\Delta_1 - \Delta_0$), and might incur additional start-up cost later, algorithm  $\text{gCHASE}_s^r$ will not change state if the decrement is small. In another word, $\text{gCHASE}_s^r$ is more stable facing the minor change in $\Delta(t)$, making it better than rCHASE on average.

\begin{figure*}[h]
\begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\textwidth]{rCHASE_up.png}  
    	\caption*{\rev{(a) On one hand, if $s_{\tau - 1}$ is 0 and $\Delta(\tau)$ is increasing slowly ($\Delta_1$), the algorithm $\text{gCHASE}_s^r$
    	will set $s_{\tau}$ to be 0 with high probability. In contrast, rCHASE will set $s_\tau$ to be 1. In such case, the cost of rCHASE will be higher than that of $\text{gCHASE}_s^r$, by the amount of $\beta - \Delta_1 + \Delta_0$. On the other hand, if $\Delta(\tau)$ is increasing quickly ($\Delta_2$), then with high probability rCHASE and  $\text{gCHASE}_s^r$ will set $s_{\tau}$ to the same value.}}
    	\label{fig:r_up}
\end{minipage}
\hfill
\begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\textwidth]{rCHASE_down.png}  
    \caption*{\com{Please rewrite this caption similar to the one in (a).} (b) For $\text{gCHASE}_s^r$, if $s_{\tau - 1}$ is 1 and $\Delta(\tau)$ is decreasing slowly ($\Delta_1$), $s_{\tau}$ will be 1 with high probability. However, $s_\tau$ of rCHASE will be 0. The cost of rCHASE will not be less than the cost of $\text{gCHASE}_s^r$ when $\Delta(t)$ increases thereafter. If $\Delta(\tau)$ is decreasing quickly ($\Delta_2$), with high probability, rCHASE and $\text{gCHASE}_s^r$ will have the same behaviour.} 
    \label{fig:r_down}
\end{minipage}
\caption{Two examples of $\Delta(t)$ and behaviors of $\text{OFA}_s$, rCHASE\cite{rchase} and $\text{gCHASE}_s^r$, showing $\text{gCHASE}_s^r$ is better than rCHASE. \com{The readers may not understand the behaviors of Algorithm 3 yet, and thus it may not be clear to them why the gCHASE would have the behaviors shown in the two examples.}}
\label{fig:r_up_down}
\end{figure*}

\begin{thm}
	\label{thm:gchaser}
	The {expected} competitive ratio of $\text{gCHASE}_s^r$ (Algorithm 3) for problem \textbf{SP} is 2.
\end{thm}

\begin{proof} (Sketch)
	By relaxing the discrete states to the continuous states setting, we show that the expected cost of $\text{gCHASE}_s^r$ is equal to a continuous version $\text{cCHASE}_s^r$. Then we show that $\text{cCHASE}_s^r$ has a competitive ratio of 2 in the continuous setting with regard to the offline optimal algorithm $\text{cOPT}_{s}$. Lastly, it can be verified that the optimal cost in the discrete setting is an upper bound to the continuous one. The logical is to show
        \begin{align}
    \mathbb{E}[{\rm Cost}_{\text{gCHASE}_s^r}] = {\rm Cost}_{\text{cCHASE}_{s}^{r}} \leq 2{\rm Cost}_{\text{cOPT}_{s}} \leq 2{\rm Cost}_{\text{OFA}_s}.
\end{align}

	See Appendix \ref{pro:ran} for the complete proof.
\end{proof}

\textbf{Remark:} 1). We improve the randomized algorithm in \cite{rchase} by taking the momentarily change of $\Delta(t)$ into consideration. 2). The original ideas of $\text{gCHASE}_s^r$ appeared in \cite{oco} and \cite{disc}. However, their algorithms are based on continuously updated probability distribution, which is much complicated in operation. 3). In \cite{disc-ext}, Theorem 8 proves that 2 is the lower bound on expected competitive ratio of any randomized online algorithm for problem \textbf{SP}. Therefore $\text{gCHASE}_s^r$ is one of the best randomized algorithms in terms of competitive ratio.

\begin{comment}
\begin{algorithm}[tb]
	\caption{$\text{gCHASE}_s^r$}
	\begin{algorithmic}
		\label{alg-gchasesr}
		\STATE Set $s_0 \leftarrow 0$
		\FOR{$t$ from 1 to $T$}
		\STATE Compute $\Delta(t)$
		\IF{$\Delta(t)=0$}
		\STATE $s_t \leftarrow 1$
		\ELSIF{$\Delta(t)=-\beta$}
		\STATE $s_t \leftarrow 0$
		\ELSE
		\IF{$\Delta(t-1)\leq \Delta(t)$}
		\IF{$s_{t-1} = 1$}
		\STATE $s_t \leftarrow 1$
		\ELSE
		\STATE $s_t \leftarrow 0$ with probability $\frac{\Delta(t)}{\Delta(t-1)}$
		\STATE $s_t \leftarrow 1$ with probability $1-\frac{\Delta(t)}{\Delta(t-1)}$
		\ENDIF
		\ENDIF
		\ELSE
		\IF{$s_{t-1} = 0$}
		\STATE $s_t \leftarrow 0$
		\ELSE
		\STATE $s_t \leftarrow 0$ with probability $1-\frac{\beta+\Delta(t)}{\beta+\Delta(t-1)}$
		\STATE $s_t \leftarrow 1$ with probability $\frac{\beta+\Delta(t)}{\beta+\Delta(t-1)}$
		\ENDIF
		\ENDIF
	    \RETURN $s_t$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}
\end{comment}



